How to Bake Quantum into Your Pet Petri Nets and Have Your Net Theory Too

Petri nets have found widespread use among many application domains, not least due to their human-friendly graphical syntax for the composition of interacting distributed and asynchronous processes and services, based in partial-order dependencies and concurrent executions. Petri nets also come with abstract semantics, and mathematical methods for compositional synthesis, structural checks and behavioural analysis. These have led to the use of various kinds of nets for real-time, distributed and parallel programming languages, software and services systems, with a view to their interfaces and interaction protocols. These affordances make Petri nets invaluable for distributed software architecture approaches focused on components, their mutual dependencies and environment-facing interactions. Quantum computing -- and in particular quantum software engineering -- is in its infancy and could benefit from the accumulated insights of software architecture research and of net theory, its methods, and its applications. In this paper, we establish a connection between Petri nets and quantum systems, such that net theory and the component architecture of nets may help in the synthesis and analysis of abstract software models and their interface protocols in hybrid classical-and-quantum programming languages and services systems. We leverage some insights from net formalisms for software specification for a versatile recipe to bake quantum into extant Petri net flavours, and prove universality and compositionality of Petri nets for quantum programming.

==> figures/FigDoubleSlitNoMatrix.tex <==
\begin{figure}[htb]
\centering
\includegraphics[width=0.5\textwidth]{figures/FigDoubleSlitPNLegend.png}
~~~~~
\raisebox{1.5cm}{
\begin{tikzpicture}[scale=1]
                                       \draw(5,8) node(A){$A$};
                       \draw(3.8,7.7) node{$a_l,u$};
                \draw(2.4,6.7) node{$l,s$};
                        \draw(4.35,7.2) node{$b_l,v$};                       
       \draw(3,7) node(L){$L$};        \draw(5,7) node(B){$B$};
                       \draw(3.8,6.25) node{$c_l,w$};
\draw(2,6) node(G){$G$};               \draw(5,6) node(C){$C$};
                       \draw(3.8,5.65) node{$a_r,u$};
                       \draw(4.35,5.2) node{$b_r,v$};                       
       \draw(3,5) node(R){$R$};        \draw(5,5) node(D){$D$};
                \draw(2.4,5.1) node{$r,s$};
                       \draw(3.8,4.2) node{$c_r,w$};                
                                       \draw(5,4) node(E){$E$};
\draw[thick,->] (G) -- (L) -- (A) edge[loop right]node{$a,1$} (A);
\draw[thick,->] (G) -- (R) -- (E) edge[loop right]node{$e,1$} (E);
\draw[thick,->] (L) -- (B) edge[loop right]node{$b,1$} (B);
\draw[thick,->] (L) -- (C) edge[loop right]node{$c,1$} (C);
\draw[thick,->] (R) -- (C);
\draw[thick,->] (R) -- (D) edge[loop right]node{$d,1$} (D);
\draw[thick,->] (R) -- (E) edge[loop right]node{$e,1$} (E);
\end{tikzpicture}
} % END RAISEBOX
\centering
\caption{\label{fig:DoubleSlit} {\em Quantum interference in a simplified particle system model of the double-slit experiment.}
\newline
{\em Left:} For any $N\in\mathbb{N}^+$, the PTN carries $N$ tokens on place $G$, only, in its initial marking. This is a live system net. Every transition can fire at least once (the net is $L_1$-live). Moreover, one of the transitions $a$ through $e$ will eventually keep firing (there is no dead marking). When weighting its transitions with classical rates, the PTN becomes an SPN of a bullet scattering. With quantum rates, it is a QPTN representing a photon scattering in a simplified double-slit experiment model. Rates not shown default to $1$.
\newline
{\em Right:} The reachability graph (RG) for N=1. With edge weights, it becomes the weighted reachability graph of the SPN or QPTN to the left.
%
All PTN states remain reachable in the SPN. 
For the SPN, markings in $A,B,D$ and $E$ are equiprobable at $1/6$. $C$ attracts tokens from both slits with twice the probability, $1/3$.
%
For the QPN, the probabilities for reaching $A,B,D$ and $E$ remain equiprobable. However surprisingly, the probability of reaching $C$ is zero due to quantum wave interference modeled by the complex rates. These can cancel each other before taking a measurement. $C$ is not reachable in the $QPTN$. Transition $c$ is dead (the net is no longer $L_1$-live). However, neither do tokens magically disappear, nor does the net have a dead marking: one of $a,b,d$ or $e$ will keep firing with probability $1/4$.
}
\end{figure}

